Underwater Image Restoration Through a Prior Guided Hybrid Sense Approach and Extensive Benchmark Analysis

Underwater imaging grapples with challenges from light-water interactions, leading to color distortions and reduced clarity. In response to these challenges, we propose a novel Color Balance Prior \textbf{Guided} \textbf{Hyb}rid \textbf{Sens}e \textbf{U}nderwater \textbf{I}mage \textbf{R}estoration framework (\textbf{GuidedHybSensUIR}). This framework operates on multiple scales, employing the proposed \textbf{Detail Restorer} module to restore low-level detailed features at finer scales and utilizing the proposed \textbf{Feature Contextualizer} module to capture long-range contextual relations of high-level general features at a broader scale. The hybridization of these different scales of sensing results effectively addresses color casts and restores blurry details. In order to effectively point out the evolutionary direction for the model, we propose a novel \textbf{Color Balance Prior} as a strong guide in the feature contextualization step and as a weak guide in the final decoding phase. We construct a comprehensive benchmark using paired training data from three real-world underwater datasets and evaluate on six test sets, including three paired and three unpaired, sourced from four real-world underwater datasets. Subsequently, we tested 14 traditional and retrained 23 deep learning existing underwater image restoration methods on this benchmark, obtaining metric results for each approach. This effort aims to furnish a valuable benchmarking dataset for standard basis for comparison. The extensive experiment results demonstrate that our method outperforms 37 other state-of-the-art methods overall on various benchmark datasets and metrics, despite not achieving the best results in certain individual cases. The code and dataset are available at \href{https://github.com/CXH-Research/GuidedHybSensUIR}{https://github.com/CXH-Research/GuidedHybSensUIR}.

==> figtex/nonRefMetric_cmp.tex <==
\begin{figure*}[ht]
    \begin{minipage}[b]{1.0\linewidth}
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_177/2016TIP_minimum_information_uieb_177_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.503 / \textbf{3.72}}}
            % \vspace{-2mm}
            % \centerline{{\scriptsize UCIQE: 0.503}}
            % \vspace{-2mm}
            % \centerline{{\scriptsize UIQM: \textbf{3.72}}}
        \end{minipage}   
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_177/ADPCC_uieb_177_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.494 / 3.01}}
            % \vspace{-2mm}
            % \centerline{{\scriptsize UCIQE:  0.494}}
            % \vspace{-2mm}
            % \centerline{{\scriptsize UIQM: 3.01}}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_177/GBdehazingRCorrection_uieb_177_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.456 / 3.25}}
            % \vspace{-2mm}
            % \centerline{{\scriptsize UCIQE:  0.456}}
            % \vspace{-2mm}
            % \centerline{{\scriptsize UIQM: 3.25}}
        \end{minipage}   
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_177/HLRP_uieb_177_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.470 / 3.37}}
            % \vspace{-2mm}
            % \centerline{{\scriptsize UCIQE: 0.470}}
            % \vspace{-2mm}
            % \centerline{{\scriptsize UIQM: 3.37}}
        \end{minipage}  
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_177/Sea-thru_uieb_177_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize \textbf{0.507} / 3.56}}
            % \vspace{-2mm}
            % \centerline{{\scriptsize UCIQE: \textbf{0.507}}}
            % \vspace{-2mm}
            % \centerline{{\scriptsize UIQM: 3.56}}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_177/CIEUI_uieb_177_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.413 / 2.76}}
            % \vspace{-2mm}
            % \centerline{{\scriptsize UCIQE: 0.413}}
            % \vspace{-2mm}
            % \centerline{{\scriptsize UIQM: 2.76}}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_177/IBLA_uieb_177_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.432 / 2.93}}
            % \vspace{-2mm}
            % \centerline{{\scriptsize UCIQE: 0.432}}
            % \vspace{-2mm}
            % \centerline{{\scriptsize UIQM: 2.93}}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_177/model16_uieb_177_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.454 / 2.82}}
            % \vspace{-2mm}
            % \centerline{{\scriptsize UCIQE: 0.454}}
            % \vspace{-2mm}
            % \centerline{{\scriptsize UIQM: 2.82}}
        \end{minipage}
    \end{minipage}

    \begin{minipage}[b]{1.0\linewidth}
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_26/2016TIP_minimum_information_uieb_26_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.503 / 3.67}}
            % \vspace{-2mm} \centerline{{\scriptsize UCIQE: 0.503}}
            % \vspace{-2mm} \centerline{{\scriptsize UIQM: 3.67}}
        \end{minipage}   
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_26/ADPCC_uieb_26_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.447 / 3.77}}
            % \vspace{-2mm} \centerline{{\scriptsize UCIQE: 0.447}}
            % \vspace{-2mm} \centerline{{\scriptsize UIQM: 3.77}}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_26/GBdehazingRCorrection_uieb_26_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.357 / \textbf{3.80}}}
            % \vspace{-2mm} \centerline{{\scriptsize UCIQE: 0.357}}
            % \vspace{-2mm} \centerline{{\scriptsize UIQM: \textbf{3.80}}}
        \end{minipage}   
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_26/HLRP_uieb_26_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize \textbf{0.534} / 2.34}}
            % \vspace{-2mm} \centerline{{\scriptsize UCIQE: \textbf{0.534}}}
            % \vspace{-2mm} \centerline{{\scriptsize UIQM: 2.34}}
        \end{minipage}  
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_26/Sea-thru_uieb_26_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.415 / 3.75}}
            % \vspace{-2mm} \centerline{{\scriptsize UCIQE: 0.415}}
            % \vspace{-2mm} \centerline{{\scriptsize UIQM: 3.75}}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_26/CIEUI_uieb_26_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.381 / 3.64}}
            % \vspace{-2mm} \centerline{{\scriptsize UCIQE: 0.381}}
            % \vspace{-2mm} \centerline{{\scriptsize UIQM: 3.64}}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_26/IBLA_uieb_26_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.470 / 1.22}}
            % \vspace{-2mm} \centerline{{\scriptsize UCIQE: 0.470}}
            % \vspace{-2mm} \centerline{{\scriptsize UIQM: 1.22}}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_26/model16_uieb_26_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.430 / 3.56}}
            % \vspace{-2mm} \centerline{{\scriptsize UCIQE: 0.430}}
            % \vspace{-2mm} \centerline{{\scriptsize UIQM: 3.56}}
        \end{minipage}
    \end{minipage}

    \begin{minipage}[b]{1.0\linewidth}
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_18/2016TIP_minimum_information_uieb_18_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.454 / 3.46}}
            % \vspace{-2mm} \centerline{{\scriptsize UCIQE: 0.454}}
            % \vspace{-2mm} \centerline{{\scriptsize UIQM: 3.46}}
        \end{minipage}   
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_18/ADPCC_uieb_18_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.459 / 2.36}}
            % \vspace{-2mm} \centerline{{\scriptsize UCIQE: 0.459}}
            % \vspace{-2mm} \centerline{{\scriptsize UIQM: 2.36}}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_18/GBdehazingRCorrection_uieb_18_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.414 / 2.62}}
            % \vspace{-2mm} \centerline{{\scriptsize UCIQE: 0.414}}
            % \vspace{-2mm} \centerline{{\scriptsize UIQM: 2.62}}
        \end{minipage}   
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_18/HLRP_uieb_18_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.376 / 3.61}}
            % \vspace{-2mm} \centerline{{\scriptsize UCIQE: 0.376}}
            % \vspace{-2mm} \centerline{{\scriptsize UIQM: 3.61}}
        \end{minipage}  
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_18/Sea-thru_uieb_18_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize \textbf{0.471} / \textbf{3.71}}}
            % \vspace{-2mm} \centerline{{\scriptsize UCIQE: \textbf{0.471}}}
            % \vspace{-2mm} \centerline{{\scriptsize UIQM: \textbf{3.71}}}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_18/CIEUI_uieb_18_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.386 / 2.37}}
            % \vspace{-2mm} \centerline{{\scriptsize UCIQE: 0.386}}
            % \vspace{-2mm} \centerline{{\scriptsize UIQM: 2.37}}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_18/IBLA_uieb_18_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.375 / 1.77}}
            % \vspace{-2mm} \centerline{{\scriptsize UCIQE: 0.375}}
            % \vspace{-2mm} \centerline{{\scriptsize UIQM: 1.77}}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.119\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/nonRefMetric_cmp/uieb_18/model16_uieb_18_img_.png}}
            \vspace{-2mm}
            \centerline{{\scriptsize 0.328 / 3.65}}
            % \vspace{-2mm} \centerline{{\scriptsize UCIQE: 0.328}}
            % \vspace{-2mm} \centerline{{\scriptsize UIQM: 3.65}}
        \end{minipage}
    \end{minipage}

    \caption{\hl{Illustrative examples demonstrating the inconsistencies in UCIQE and UIQM Performance. The top metrics are highlighted in bold. Although a higher score in these metrics is intended to indicate superior image quality, the images with higher scores or rankings in this figure paradoxically exhibit poor quality.}}
    \label{fig:nonRefMetricCmp}
\end{figure*}

==> figtex/overall_arch.tex <==
\begin{figure*}[ht]
\centering
% \vspace*{-0.05in}
\includegraphics[width=\textwidth]{figs/overall_arch.pdf}
\caption{The overall architecture of the proposed GuidedHybSensUIR.}
\label{fig:overall}
\end{figure*}


==> tabletex/1_quan.tex <==
\begin{table*}[ht]
\caption{Quantitative comparison on the paired test sets UIEB, EUVP and LSUI. The table is organized with traditional methods listed in the upper section and deep learning methods detailed in the lower section. Due to the large margin between the metrics of the deep learning methods and the traditional methods, the highest-performing results and the second-best results are highlighted in bold and underlined, respectively, within each section for better comparison.}
\adjustbox{width=\textwidth}{%
\begin{tabular}{lrrrrrrrrrrrrrr}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Computational Cost}} & \multicolumn{4}{c}{\textbf{UIEB}}                         & \multicolumn{4}{c}{\textbf{EUVP}}                        & \multicolumn{4}{c}{\textbf{LSUI}}                        \\ \cmidrule(lr){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-11}  \cmidrule(lr){12-15}
                        & MACs(G)$\downarrow$ & Params(M)$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & UCIQE$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & UCIQE$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & UCIQE$\uparrow$ \\ \midrule
\textbf{WCID} \cite{chiang2011underwater}                    & \multicolumn{1}{c}{-}                      & \multicolumn{1}{c}{-}                  & 11.65          & 0.322          & 0.424           & 0.453           & 12.93          & 0.270          & 0.480           & 0.491           & 12.38          & 0.285          & 0.444           & 0.450           \\
\textbf{Fusion} \cite{ancuti2012enhancing}                  & \multicolumn{1}{c}{-}                      & \multicolumn{1}{c}{-}                  & 15.00          & 0.726          & 0.373           & 0.342           & 16.07          & 0.703          & 0.372           & 0.411           & 16.09          & 0.756          & 0.324           & 0.394           \\
\textbf{GBD\&RC} \cite{li2016single}                 & \multicolumn{1}{c}{-}                      & \multicolumn{1}{c}{-}                  & 12.35          & 0.625          & 0.446           & \underline{0.509}     & 14.20          & 0.598          & 0.449           & \textbf{0.575}  & 13.59          & 0.648          & 0.460           & \textbf{0.547}  \\
\textbf{min\_info\_loss} \cite{li2016underwater}          & \multicolumn{1}{c}{-}                      & \multicolumn{1}{c}{-}                  & 17.13    & 0.783          & 0.327           & \textbf{0.544}  & 15.23          & 0.643          & 0.439           & 0.497           & 16.41          & 0.720          & 0.382           & 0.498           \\
\textbf{IBLA} \cite{peng2017underwater}                    & \multicolumn{1}{c}{-}                      & \multicolumn{1}{c}{-}                  & 15.93          & 0.710          & 0.291           & 0.447           & \textbf{18.91} & \underline{0.710}    & \textbf{0.319}  & 0.483           & 16.95          & 0.721          & 0.331           & 0.461           \\
\textbf{Sea-thru} \cite{akkaynak2019sea}                 & \multicolumn{1}{c}{-}                      & \multicolumn{1}{c}{-}                  & 13.82          & 0.580          & 0.421           & 0.502           & 12.72          & 0.499          & 0.496           & \underline{0.518}     & 12.91          & 0.505          & 0.501           & \underline{0.518}     \\
\textbf{UNTV} \cite{xie2021variational}                    & \multicolumn{1}{c}{-}             & \multicolumn{1}{c}{-}               & 16.46 & 0.669          & 0.420           & 0.436           & \underline{17.63}    & 0.611          & 0.335           & 0.481           & \textbf{18.36} & 0.660          & 0.376           & 0.449           \\
\textbf{HLRP} \cite{zhuang2022underwater}                    & \multicolumn{1}{c}{-}                      & \multicolumn{1}{c}{-}                  & 13.30          & 0.259          & 0.364           & 0.476           & 11.41          & 0.186          & 0.500           & 0.509           & 12.96          & 0.221          & 0.429           & 0.503           \\
\textbf{MLLE} \cite{zhang2022underwater}                    & \multicolumn{1}{c}{-}                      & \multicolumn{1}{c}{-}                  & \textbf{18.74} & 0.814          & 0.234           & 0.444           & 15.14          & 0.633          & \underline{0.323}     & 0.474           & 17.87          & 0.730          & \textbf{0.278}  & 0.457           \\
\textbf{ROP} \cite{liu2022rank}                     & \multicolumn{1}{c}{-}                      & \multicolumn{1}{c}{-}                  & 18.48          & \textbf{0.849} & \textbf{0.209}  & 0.454           & 15.34          & \textbf{0.714} & 0.343           & 0.441           & 17.38          & \textbf{0.806} & \underline{0.281}     & 0.448           \\
\textbf{ROP+} \cite{liu2022rank}                    & \multicolumn{1}{c}{-}                      & \multicolumn{1}{c}{-}                  & 15.88          & 0.776          & 0.287           & 0.449           & 13.46          & 0.613          & 0.393           & 0.450           & 14.51          & 0.692          & 0.354           & 0.443           \\
\textbf{ADPCC} \cite{zhou2023underwater}                   & \multicolumn{1}{c}{-}                      & \multicolumn{1}{c}{-}                  & 17.33          & 0.819          & 0.219           & 0.485           & 15.20          & 0.692          & 0.349           & 0.495           & 16.20          & \underline{0.763}    & 0.299           & 0.481           \\
\textbf{ICSP} \cite{hou2023non}                    & \multicolumn{1}{c}{-}                      & \multicolumn{1}{c}{-}                  & 12.04          & 0.599          & 0.552           & 0.408           & 11.73          & 0.522          & 0.413           & 0.443           & 11.96          & 0.583          & 0.508           & 0.399           \\
\textbf{WWPF} \cite{zhang2023underwater}                    & \multicolumn{1}{c}{-}                      & \multicolumn{1}{c}{-}                  & \underline{18.60}    & \underline{0.822}    & \underline{0.218}     & 0.446           & 15.95          & 0.648          & 0.337           & 0.467           & \underline{17.90}    & 0.739          & 0.283           & 0.456           \\ \midrule
\textbf{UGAN} \cite{fabbri2018enhancing}                    & 19.82                 & 57.17                   & 21.52          & 0.804          & 0.189           & 0.427           & 23.30          & 0.815          & 0.220           & \textbf{0.442}  & 24.22          & 0.840          & 0.191           & \textbf{0.433}  \\
\textbf{WaterNet} \cite{li2019underwater}                & 71.42                 & 1.09                    & 22.82          & 0.907          & 0.125           & \underline{0.436}     & 24.12          & 0.839          & 0.222           & 0.426           & 25.25          & 0.877          & 0.164           & 0.418           \\
\textbf{UWCNN} \cite{li2020underwater}                   & \textbf{2.61}         & \textbf{0.04}           & 18.44          & 0.844          & 0.203           & 0.367           & 23.49          & 0.830          & 0.231           & 0.407           & 21.73          & 0.844          & 0.228           & 0.360           \\
\textbf{Shallow-UWNet} \cite{naik2021shallow}           & 21.63                 & \underline{0.22}              & 18.30          & 0.846          & 0.206           & 0.355           & 23.59          & 0.832          & 0.228           & 0.401           & 21.91          & 0.846          & 0.233           & 0.352           \\
\textbf{Ucolor} \cite{li2021underwater}                  & 1002.00               & 105.51                  & 18.37          & 0.814          & 0.221           & 0.370           & 23.72          & 0.828          & 0.205           & 0.408           & 21.30          & 0.821          & 0.225           & 0.362           \\
\textbf{CLUIE-Net} \cite{li2022beyond}                & 31.13                                 & 13.40                                   & 19.95          & 0.874          & 0.168           & 0.403           & 24.85          & 0.844          & 0.186           & 0.415           & 23.57          & 0.864          & 0.175           & 0.396           \\
\textbf{PUIE-Net} \cite{fu2022uncertainty}                 & 30.09                                 & 1.40                                    & 21.04          & 0.877          & 0.136           & 0.370           & 20.48          & 0.784          & 0.270           & 0.391           & 22.07          & 0.864          & 0.191           & 0.378           \\
\textbf{STSC} \cite{wang2022semantic}                     & 204.84                                & 32.92                                   & 21.20          & 0.820          & 0.183           & 0.415           & 25.08          & 0.844          & 0.176           & 0.414           & 24.26          & 0.851          & 0.181           & 0.402           \\
\textbf{TACL} \cite{liu2022twin}                     & 120.03                                & 28.29                                   & 19.83          & 0.761          & 0.222           & 0.427           & 20.99          & 0.782          & 0.213           & 0.440           & 22.97          & 0.828          & 0.176           & \textbf{0.433}  \\
\textbf{UIE-WD} \cite{ma2022wavelet}                   & 51.38                                 & 14.49                                   & 20.28          & 0.848          & 0.198           & 0.407           & 17.80          & 0.760          & 0.292           & 0.440           & 19.23          & 0.803          & 0.284           & 0.410           \\
\textbf{URSCT} \cite{ren2022reinforced}                   & 18.11                                 & 11.26                                   & 22.77          & 0.915          & 0.120           & 0.432           & \underline{25.74}    & \textbf{0.855} & 0.180           & 0.425           & \underline{25.87}    & \textbf{0.883} & \underline{0.146}     & 0.417  \\
\textbf{USUIR} \cite{fu2022unsupervised}                   & 14.81                                 & 0.23                                    & 22.48          & 0.907          & 0.124           & 0.427           & 21.94    & 0.810 & 0.239           & 0.408           & 23.75    & 0.860 & 0.184     & 0.412           \\
\textbf{CCMSRNet} \cite{qi2023deep}                 & 43.60                                 & 21.13                                   & 17.04          & 0.790          & 0.322           & 0.424           & 17.77          & 0.720          & 0.381           & 0.436  & 18.54          & 0.788          & 0.352           & 0.430           \\
\textbf{DeepWaveNet} \cite{sharma2023wavelength}              & 18.15                                 & 0.28                                    & 21.55 & 0.904          & 0.143           & 0.424           & 23.41          & 0.836          & 0.204     & 0.426           & 23.81          & 0.870          & 0.177           & 0.415           \\
\textbf{GUPDM} \cite{mu2023generalized}                   & 95.80                                 & 1.49                                    & 22.13          & 0.903    & 0.131     & 0.427  & 24.79          & 0.847    & 0.184           & 0.431           & 25.33          & 0.877          & 0.150           & 0.420           \\
\textbf{MBANet} \cite{xue2023investigating}                  & 11.30                                 & 0.52                                    & 19.58          & 0.800          & 0.209           & 0.414           & 23.76          & 0.819    & 0.225           & 0.436           & 23.02          & 0.843          & 0.210           & 0.420           \\
\textbf{$ \mathbf{NU^2Net}$ } \cite{guo2023underwater}                  & 10.49                                 & 3.15                                    & 19.99          & 0.850          & 0.196           & 0.390           & 21.51          & 0.810          & 0.308           & 0.419           & 22.13          & 0.872          & 0.243           & 0.396           \\
\textbf{PUGAN} \cite{cong2023pugan}                    & 75.40                                 & 101.19                                  & 20.52          & 0.812          & 0.216           & 0.418           & 22.58          & 0.820          & 0.212           & 0.425           & 23.14          & 0.836          & 0.216           & 0.413           \\
\textbf{Semi-UIR} \cite{huang2023contrastive}                 & 72.88                                 & 3.31                                    & \textbf{23.64} & 0.888          & 0.120           & 0.428           & 24.59          & 0.821          & \underline{0.172}     & 0.424           & 25.40          & 0.843          & 0.160           & 0.419           \\
\textbf{SyreaNet} \cite{wen2023syreanet}                & 140.88                                & 29.05                                   & 22.72          & \underline{0.918}    & \underline{0.116}     & \textbf{0.442}  & 23.25          & 0.834          & 0.224           & 0.418           & 24.90          & 0.872          & 0.168           & 0.422           \\
\textbf{TUDA} \cite{wang2023domain}                     & 85.43                           & 2.73                                    & 22.72          & 0.915          & 0.118           & 0.429           & 23.73          & 0.843          & 0.207           & 0.415           & 25.52          & 0.878          & 0.154           & 0.417           \\
\textbf{U-Transformer} \cite{peng2023u}           & \underline{2.98}                            & 22.82                                   & 20.75          & 0.810          & 0.228           & 0.434           & 24.99          & 0.829          & 0.238           & 0.434           & 25.15          & 0.838          & 0.221           & 0.427           \\
\textbf{SFGNet} \cite{zhao2024toward}                  & 81.58                                 & 1.30                                    & 19.57          & 0.685          & 0.214           & 0.432           & 22.68          & 0.585          & 0.221           & \textbf{0.442}  & 22.71          & 0.653          & 0.204           & 0.426           \\
\textbf{Ours}                     & 10.05                 & 1.15                    & \underline{23.63}    & \textbf{0.923} & \textbf{0.100}  & 0.433           & \textbf{25.75} & \underline{0.847}    & \textbf{0.111}  & \underline{0.441}     & \textbf{26.39} & \underline{0.880}    & \textbf{0.098}  & \underline{0.432}     \\
\bottomrule
\end{tabular}%
}
\label{tab:quan1}
\end{table*}


==> tabletex/2_userstudy.tex <==
\begin{table}[ht]
\caption{Comparison of user study scores for five deep learning-based methods. Traditional methods' scores are significantly lower than deep learning methods and are omitted due to space constraints.}
\adjustbox{width=0.48\textwidth}{%
\begin{tabular}{lrrrrrr}
\toprule
Method & Ours          & Semi-UIR & GUPDM & WaterNet & TUDA & URSCT \\
\midrule
UIEB   & \textbf{4.63} & 4.50     & 4.08  & 3.78     & 3.65 & 2.75          \\
EUVP   & \textbf{4.70} & 4.30     & 4.20  & 4.15     & 3.95 & 4.13          \\
LSUI   & \textbf{4.58} & 4.43     & 4.30  & 4.10     & 4.05 & 3.60          \\
Mean   & \textbf{4.63} & 4.41     & 4.19  & 4.01     & 3.88 & 3.49  \\
URSCT needs update
\bottomrule
\end{tabular}
}
\label{tab:userstudy}
\end{table}

==> tabletex/3_ablation.tex <==
\begin{table}[ht]
\centering
\caption{Quantitative results of ablation studies. The results underscore the critical contributions of each component to the overall performance metrics.}
\adjustbox{width=0.4\textwidth}{%
\begin{tabular}{lrrrr}
\toprule
Method       & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & UCIQE$\uparrow$ \\
\midrule
W/O Prior    & 24.97          & 0.881          & 0.107          & 0.427          \\
W/O FC       & 24.68          & 0.880          & 0.110          & 0.418          \\
W/O Prior+FC & 24.67          & 0.877          & 0.114          & 0.422          \\
W/O DR       & 24.78          & 0.876          & 0.117          & 0.422          \\
W/O SH       & 24.81          & 0.880          & 0.108          & 0.419          \\
Full Model   & \textbf{25.25} & \textbf{0.883} & \textbf{0.103} & \textbf{0.435}   \\
\bottomrule
\end{tabular}
}
\label{tab:ablation}
\end{table}

==> tabletex/3_ablation_v2.tex <==
\begin{table}[ht]
\centering
\caption{Quantitative results of ablation studies. The results underscore the critical contributions of each component to the overall performance metrics.}
\adjustbox{width=\columnwidth}{%
\begin{tabular}{ccccrrrr}
\toprule
Prior & FC & DR & SH       & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & UCIQE$\uparrow$ \\
\midrule
\tiny{\XSolidBold}     & \Checkmark  & \Checkmark  & \Checkmark  & 24.97          & 0.881          & 0.107          & 0.427          \\
\Checkmark     & \tiny{\XSolidBold}  & \Checkmark  & \Checkmark  & 24.68          & 0.880          & 0.110          & 0.418          \\
\tiny{\XSolidBold}     & \tiny{\XSolidBold}  & \Checkmark  & \Checkmark  & 24.67          & 0.877          & 0.114          & 0.422          \\
\Checkmark     & \Checkmark  & \tiny{\XSolidBold}  & \Checkmark  & 24.78          & 0.876          & 0.117          & 0.422          \\
\Checkmark     & \Checkmark  & \Checkmark  & \tiny{\XSolidBold}  & 24.81          & 0.880          & 0.108          & 0.419          \\
\Checkmark     & \Checkmark  & \Checkmark  & \Checkmark  & \textbf{25.25} & \textbf{0.883} & \textbf{0.103} & \textbf{0.435}   \\
\bottomrule
\end{tabular}
}
\label{tab:ablation}
\end{table}
